Determining the Efficacy of Different Parameterizations of the z-expansion

We develop a methodology to test the accuracy of lattice extrapolations of the form factors in B decays only using experimental data. We test this methodology by comparing the BGL parameterization proposed by Boyd, Grinstein, and Lebed (1996) and the BCL parameterization proposed by Bourrely Caprini and Lellouch (2008) in the context of $B \rightarrow \pi \ell \nu$. Our results suggest that the BCL parameterization is a slightly better predictor of the low $q^2$ region than the BGL parameterization and that this methodology can be extended to other decays such as $B\rightarrow D\ell \nu$.

==> Lattice Proceedings/Tex/oldcomparison.tex <==
\section{Comparison of Two Parameterizations at equal number of parameters}
We examined in detail the BGL and BCL parameterizations of the vector form factor $f_+(q^2)$ for the decay $B \rightarrow \pi \ell \nu$ at 3 and 4 parameters for both the BCL and BGL expansions. These two orders were chosen as they provide an interesting look at the behavior of the two parameterizations of the form factors.
\subsection{Comparison of Lattice Region}

\begin{figure}[t]
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_3_parameter_fit__range_17_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_3_parameter_fit__range_17_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_4_parameter_fit__range_17_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_3_parameter_fit__range_17_26.png}

\caption{fits to experimental data fitted $q^2 > 17 ~\text{GeV}^2$.}
\label{fig:expfit17264}
\end{figure}
The 3 and 4 parameter fits corresponding to the lattice region is in both cases over estimates the partial branching fractions outside of the lattice region \fref{fig:expfit17264}. In fact the BCL fit appears to overestimate the partial branching fractions more than the BGL expansion for 3 parameters but this is inverted for 4 parameters. This is verified in comparing the predictive measures $X_p^2$ (see \fref{tab:Xp2vals}). 
\begin{table}
\begin{tabular}{| c | c | c | c |}
\hline
coefs & type & 17 - 26.4 GeV$^2$ & 15 - 26.4 GeV$^2$\\ \hline
3 & BGL & 17.59 & 3.23 \\ \hline
3 & BCL & 48.5   &  3.34 \\ \hline
4 & BGL & 897    & 1.90 \\ \hline
4 & BCL & 156    & 4.33 \\ \hline
\end{tabular}
\caption{$X_p^2$ for a 3 and 4 parameter BGL and BCL expansions in the lattice and near lattice regions}
\label{tab:Xp2vals}
\end{table}
\begin{figure}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_3_parameter_fit__range_15_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_3_parameter_fit__range_15_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_4_parameter_fit__range_15_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_4_parameter_fit__range_15_26.png}
\caption{fits to experimental data fitted $q^2 > 15 ~\text{GeV}^2$.}
\label{fig:expfit15264}
\end{figure}


==> Tex/oldcomparison.tex <==
\section{Comparison of Two Parameterizations at equal number of parameters}
We examined in detail the BGL and BCL parameterizations of the vector form factor $f_+(q^2)$ for the decay $B \rightarrow \pi \ell \nu$ at 3 and 4 parameters for both the BCL and BGL expansions. These two orders were chosen as they provide an interesting look at the behavior of the two parameterizations of the form factors.
\subsection{Comparison of Lattice Region}

\begin{figure}[t]
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_3_parameter_fit__range_17_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_3_parameter_fit__range_17_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_4_parameter_fit__range_17_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_3_parameter_fit__range_17_26.png}

\caption{fits to experimental data fitted $q^2 > 17 ~\text{GeV}^2$.}
\label{fig:expfit17264}
\end{figure}
The 3 and 4 parameter fits corresponding to the lattice region is in both cases over estimates the partial branching fractions outside of the lattice region \fref{fig:expfit17264}. In fact the BCL fit appears to overestimate the partial branching fractions more than the BGL expansion for 3 parameters but this is inverted for 4 parameters. This is verified in comparing the predictive measures $X_p^2$ (see \fref{tab:Xp2vals}). 
\begin{table}
\begin{tabular}{| c | c | c | c |}
\hline
coefs & type & 17 - 26.4 GeV$^2$ & 15 - 26.4 GeV$^2$\\ \hline
3 & BGL & 17.59 & 3.23 \\ \hline
3 & BCL & 48.5   &  3.34 \\ \hline
4 & BGL & 897    & 1.90 \\ \hline
4 & BCL & 156    & 4.33 \\ \hline
\end{tabular}
\caption{$X_p^2$ for a 3 and 4 parameter BGL and BCL expansions in the lattice and near lattice regions}
\label{tab:Xp2vals}
\end{table}
\begin{figure}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_3_parameter_fit__range_15_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_3_parameter_fit__range_15_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BGL_4_parameter_fit__range_15_26.png}
\includegraphics[width=0.25\textwidth]{Graphics/experimental_fit_nolegend_BCL_4_parameter_fit__range_15_26.png}
\caption{fits to experimental data fitted $q^2 > 15 ~\text{GeV}^2$.}
\label{fig:expfit15264}
\end{figure}

